KiDS+VIKING+GAMA: Halo occupation distributions and correlations of satellite numbers with a new halo model of the galaxy-matter bispectrum for galaxy-galaxy-galaxy lensing

Halo models and halo occupation distributions (HODs) are important tools to model the galaxy and matter distribution. We present and assess a new method for constraining the parameters of HODs using the gravitational lensing shear around galaxy pairs, galaxy-galaxy-galaxy-lensing (G3L). In contrast to galaxy-galaxy-lensing, G3L is sensitive to correlations between the per-halo numbers of galaxies from different populations. We use G3L to probe these correlations and test the default hypothesis that they are negligible. We derive a halo model for G3L and validate it with realistic mock data from the Millennium Simulation and a semi-analytic galaxy model. Then, we analyse public data from the Kilo-Degree Survey (KiDS), the VISTA Infrared Kilo-Degree Galaxy Survey (VIKING) and data from the Galaxy And Mass Assembly Survey (GAMA) to infer the HODs of galaxies at $z<0.5$ in five different stellar mass bins between $10^{8.5}h^{-2} M_\odot$ and $10^{11.5}h^{-2} M_\odot$ and two colours (red and blue), as well as correlations between satellite numbers. The analysis recovers the true HODs in the simulated data within the $68\%$ credibility range. The inferred HODs vary significantly with colour and stellar mass. There is also strong evidence ($>3\sigma$) for correlations, increasing with halo mass, between the numbers of red and blue satellites and galaxies with stellar masses below $10^{10} \Msun. Possible causes of these correlations are the selection of similar galaxies in different samples, the survey flux limit, or physical mechanisms like a fixed ratio between the satellite numbers of distinct populations. The decorrelation for halos with smaller masses is probably an effect of shot noise by low-occupancy halos. The inferred HODs can be used to complement galaxy-galaxy-lensing or galaxy clustering HOD studies or as input to cosmological analyses and improved mock galaxy catalogues.

==> Submit - ArXiV/myDef.tex <==
\newcommand{\Map}{\mathcal{M}}
\newcommand{\Nap}{\mathcal{N}}
\newcommand{\Mperp}{\Map_{\perp}}

\newcommand{\NMap}{\expval{\Nap\Map}}
\newcommand{\NNMap}{\expval{\Nap\Nap\Map}}
\newcommand{\NNMperp}{\expval{\Nap\Nap\Mperp}}
\newcommand{\NMapMap}{\expval{\Nap\Map^2}}

%\newcommand{\a}{^a}
%\newcommand{\b}{^b}
%\newcommand{\ab}{^{ab}}
\newcommand{\NNM}[2]{\expval{\Nap^{#1}\Nap^{#2}\Map}}

\newcommand{\G}{\mathcal{G}}
\newcommand{\Gtilde}{\tilde{\mathcal{G}}}
\newcommand{\I}{\mathrm{i}}
\newcommand{\varthetavec}{\vb*{\vartheta}}
\newcommand{\thetavec}{\vb*{\theta}}
\newcommand{\alphavec}{\vb*{\alpha}}
\newcommand{\ellvec}{\vb*{\ell}}
\newcommand{\yvec}{\vb*{y}}
\newcommand{\kparallel}{\vb*{k}^{\|}}
\newcommand{\kperp}{k^{\perp}}
\newcommand{\SigCrit}{\Sigma_{\textrm{crit}}}
\newcommand{\SigCritAve}{\bar{\Sigma}_{\textrm{crit}}}
\newcommand{\bggk}{\mathit{b}_{\mathrm{gg}\kappa}}
\newcommand{\Bggd}{\mathit{B}_{\mathrm{gg}\delta}}
\newcommand{\Bggdab}{\Bggd^{ab}}
\newcommand{\Bggdabh}[1]{{}_{#1}\Bggd^{ab}}
\newcommand{\Bggdaah}[1]{{}_{#1}\Bggd^{aa}}
\newcommand{\bggkab}{\bggk^{ab}}
\newcommand{\dirac}{\delta_\textrm{D}}
\newcommand{\kronecker}[2]{\delta^\textrm{K}_{#1 #2}}
\newcommand{\Msun}{{M}_{\odot}}
\newcommand{\SNR}{\text{SNR}}

\newcommand{\Ns}[1]{N_{\mathrm{sat}}^{#1}}
\newcommand{\Nc}[1]{N_{\mathrm{cen}}^{#1}}
\newcommand{\Nss}[2]{N_{\mathrm{sat}, #2}^{#1}}
\newcommand{\Ncc}[2]{N_{\mathrm{cen}, #2}^{#1}}

\newcommand{\rmg}{_\mathrm{g}}

\newcommand{\pma}[2]{_{-#1}^{+#2}}

